The On-Chain and Off-Chain Mechanisms of DAO-to-DAO Voting

Voting is the primary mechanism through which Decentralised Autonomous Organisations (DAOs) reach decisions. Although transparent, the voting process can be opaque: it can involve many interacting smart contracts. The nexus of the decision-making process can be relocated and the true voter demographic obfuscated. DAOs can also govern other DAOs, a process known as metagovernance. We present a method for identifying DAO-to-DAO metagovernance on the Ethereum blockchain. We focus on the links between DAOs and token contracts. We use a signature-matching algorithm to handle a variety of DAO frameworks and voting schemes. Once we establish token-to-DAO relationships, we gather and process voting data to produce a list of metagovernance relationships. We apply this algorithm to an initial set of sixteen DAOs and we extend the dataset as more DAOs are identified. We produce a metagovernance network with 61 DAOs and 72 metagovernance relationships. We examine three case studies that show metagovernance of various forms: strategic, decisive, and nexus, where a DAO becomes a governance hub for multiple other DAOs. We demonstrate that metagovernance obscures voting context and introduces entities driven by self-interest that can significantly influence governance. We highlight instances of metagovernance between DAOs operating on the Ethereum blockchain where current governance tools fail to reveal such dynamics. Better tools are needed to preserve the transparency-centric ethos of DAOs and mitigate risks associated with metagovernance.

==> acronyms.tex <==
\newacronym{api}{API}{application programming interface}
\newacronym{dao}{DAO}{Decentralised Autonomous Organisation}
\newacronym{eoa}{EOA}{externally-owned account}
\newacronym{roi}{RoI}{Republic of Ireland}
\newacronym{setu}{SETU}{South East Technological University}

